Online Learning Demands in Max-min Fairness

We describe mechanisms for the allocation of a scarce resource among multiple users in a way that is efficient, fair, and strategy-proof, but when users do not know their resource requirements. The mechanism is repeated for multiple rounds and a user's requirements can change on each round. At the end of each round, users provide feedback about the allocation they received, enabling the mechanism to learn user preferences over time. Such situations are common in the shared usage of a compute cluster among many users in an organisation, where all teams may not precisely know the amount of resources needed to execute their jobs. By understating their requirements, users will receive less than they need and consequently not achieve their goals. By overstating them, they may siphon away precious resources that could be useful to others in the organisation. We formalise this task of online learning in fair division via notions of efficiency, fairness, and strategy-proofness applicable to this setting, and study this problem under three types of feedback: when the users' observations are deterministic, when they are stochastic and follow a parametric model, and when they are stochastic and nonparametric. We derive mechanisms inspired by the classical max-min fairness procedure that achieve these requisites, and quantify the extent to which they are achieved via asymptotic rates. We corroborate these insights with an experimental evaluation on synthetic problems and a web-serving task.

==> _ <==
 
\section{Problem Setup}
\label{sec:setup}

In this section, we will first review fair allocation and describe \mmf, one of the most
common methods for fair allocation.
We will then describe the learning problem.

\subsection{Fair Division}

% \textbf{Fair Division:}
There are $n$ agents sharing a resource of size $1$.
Agent $i$ has an entitlement $\entitli$ to the resource, where $\entitli>0$ and
$\sum_{i=1}^n\entitli=1$.
At any given instant, let $\demtruei$ denote the true demand for user $i$,
where $\demtruei \geq 0$ for all users $i$.
Continuing with the example from Section~\ref{sec:intro},
this resource could be a compute cluster shared by $n$ users in an organisation.
The entitlements are set by the management depending on whether a user's workload consists
of time-sensitive live traffic or offline job processing, and $\demtruei$ is the amount of the
resource user $i$ needs to achieve her SLOs.
% In some use-cases $\entitli$ could denote the contribution of each
In some use cases, $\entitli$ may represent the contribution of each
agent to a federated system,  such as in universities where it could be set based on the
contribution of each research group to purchase a cluster.

In a mechanism for fair allocation, each agent reports their demand $\demi$ 
(not necessarily truthfully) to the mechanism;
the mechanism returns an allocation vector $\alloc\in\RR_+^n$, where $\alloci$ is the amount of the
resource allocated to agent $i$.
Here, $\sum_{i=1}^n \alloc_i \leq 1$.
Let $\utili:\RR_+\rightarrow\RR_+$ denote agent $i$'s utility function where $\utili(a)$ is the
value agent $i$ derives if the mechanism allocates an amount $a$ of the resource to her.
She wishes to receive resources up to
her demand, but has no value for resources beyond her demand;
therefore, her utility $\utili$ is increasing up to $\demi$,
but $\utili(a) = \utili(\demi)$ for all $a>\demi$.
Additionally, we assume that $\utili$ is Lipschitz continuous with Lipschitz constant $\Lipi$.
% \emph{(i)\, Efficiency:} 

% A mechanism for fair division should ideally satisfy the following three desiderata:
The literature on fair division typically considers three desiderata for a mechanism:
% A mechanism for fair division should ideally satisfy the following three desiderata:
\emph{(i)} efficiency,
\emph{(ii)} fairness,
\emph{(iii)} strategy-proofness.
\emph{Efficiency} means that there are no unused resources when there is an unmet demand.
% Formally, 
% let $\dem\in\RR_+^n$ be a vector of demands and $\alloc\in\RR_+^n$ be a vector
% of allocations output by a mechanism.
To define it formally,
let $\lotur, \lotor, \lotud$ be as defined below for given $\dem,\alloc\in\RR_+^n$:
% is the amount of unallocated resources in this instance,
\begin{align*}
\lotur(\alloc) = 1-\sum\nolimits_{i=1}^n \alloc_i,
% \hspace{0.1in}
\hspace{0.2in}
% \lotor(\dem,\alloc) = \sum_{i\in[n]} \max(\dem_i - \alloc_i, 0),
\lotor(\dem, \alloc) = \sum\nolimits_{i=1}^n (\alloc_i - \dem_i)^+,
\hspace{0.2in}
% \hspace{0.1in}
% \lotud(\dem,\alloc) = \sum_{i\in[n]} \max(\alloc_i - \dem_i, 0).
\lotud(\dem, \alloc) = \sum\nolimits_{i=1}^n (\dem_i  - \alloc_i)^+.
\label{eqn:lotdefn}
\numberthis
\end{align*}
Here, $y^+=\max(y, 0)$.
If $\demtrue\in\RR_+^n$ is the vector of true demands and $\alloc\in\RR_+^n$ is a vector
of allocations output by a mechanism,
then $\lotur(\alloc)$ is the amount of unallocated resources in this instance,
$\lotor(\demtrue,\alloc)$ is the sum of over-allocated resources (allocated over a
user's demand) and
$\lotud(\demtrue,\alloc)$ is the sum of unmet demands (allocated under a user's demand). 
Then, $\lotur(\alloc) + \lotor(\demtrue,\alloc)$ is the total amount of resources that are not
being used, and
$\lot(\demtrue,\alloc) = \min(\lotur(\alloc) + \lotor(\demtrue,\alloc), \lotud(\demtrue,\alloc))$
is the amount of resources that are not being used but could have been used to improve the utility
of some agent.
A mechanism is efficient if, for all $\demtrue$, and when all agents report their true
demands,  $\;\lot(\demtrue,\alloc) = 0$.
% It is not hard to see that an efficient mechanism is also Pareto-optimal, in that one user's
An efficient mechanism is Pareto-optimal, in that one user's
utility can be increased only by decreasing the utility of another.
Next, a mechanism is \emph{fair} (also known as sharing incentive or individual rationality)
if the utility a truthful user derives from an allocation is at least as
much as if she had been allocated her entitlement;
i.e., for all $i, a, d$,  $\utili(\alloc_i) \geq \utili(\entitli)$.
Recall that the allocation an agent receives depends on the demands reported by the other agents.
Finally, a mechanism is \emph{strategy-proof} if no agent benefits by misreporting their demands.
That is, consider any agent $i$ and fix the demands reported by all other agents.
Let $\alloc^\star$ be the allocation returned by the mechanism when agent $i$
reports her true demand $\demtruei$,
and $\alloc$ be the allocation vector when she reports any other demand $\dem$.
Strategy-proofness means that for any agent $i$ and for all reported demands
from other agents, $\utili(\alloc_i^\star) \geq \utili(\alloc_i)$.

Observe that the above formalism does not assume that agents' utilities are comparable;
the utilities
are used solely to specify an agent's preferences over different allocations.
Therefore, notions such as utilitarian welfare which accumulates the utilities of all agents are not
meaningful in this setting.

\subsection{Max-min Fairness}
\insertAlgoMMF
% \textbf{Max-min Fairness:}
Algorithm~\ref{alg:mmf} describes \mmf, a popular mechanism for fair division.
It allocates the demands to users whose demands are small relative to their entitlement;
for all other agents whose demands cannot be satisfied simultaneously,
it allocates in proportion to their entitlements.
The following theorem establishes that \mmfs satisfies the above desiderata;
its proof is given in Section~\ref{sec:pfmmf}, where we have also established other useful
properties of \mmfs which are used elsewhere in our analysis.

\insertprethmspacing
\begin{theorem}
\label{thm:mmf}
\emph{\mmf} (Algorithm~\ref{alg:mmf}) is efficient, fair, and strategy-proof.
\end{theorem}


As an example, consider $4$ users with equal entitlements and true
demands $\{0.1, 0.28, 0.4, 0.5\}$.
\mmfs returns the allocation $\{0.1, 0.28, 0.31, 0.31\}$.
% In contrast, had we allocated the resources equally, agent 2 will not have met her demand,
Instead, had we allocated the resources equally according to their entitlements,
i.e. $\{0.25, 0.25, 0.25, 0.25\}$, agent 2 will not have met her demand,
agents 3 and 4 will not have received as much, while agent 1 will have been
sitting on 0.15 of the resource---this is fair and (trivially) strategy-proof, but inefficient.


\subsection{Online Estimation of Demands}

% \textbf{Online Estimation of Demands:}
% We now describe the problem of learning the demands online in this setting.  
We begin
our formalism for the online learning version of the fair division problem with
a description of the environment.  
% Our formalism for the online learning version of the fair allocation problem begins with
% a description of the environment.  
We consider a multi-round setting, where,
on round $t$, agent $i$ faces a load $\volit$ with (unknown)
demand $\demtrueit$.
In order to be able to effectively learn, we need a form of 
feedback for each agent which informs us of the agent's utility, and additionally be able to
relate the loads from different time steps.
For this, we define an (unknown) \emph{payoff} function $\payoffi:\RR_+\rightarrow \RR$ for each agent
$i$, which will characterise the agent's utility function.
When user $i$ receives an allocation $\allocit$ on round $t$, she observes a reward $\Xit$.
We will consider different feedback models where these rewards can be deterministic,
in which case $\Xit=\payoffi(\allocit/\volit)$, or they can be stochastic,
in which case $\Xit$
is drawn from a $\sigmait$ sub-Gaussian distribution with mean $\payoffi(\allocit/\volit)$.
% whose expectation is $\payoffi(\allocit/\volit)$.
% 

\insertFigPayoffIllus
The payoff $\payoffi$ is a non-decreasing function of the amount of resources
allocated per unit load.
% $\payoffi$ is an increasing function and satisfies $\payoffi(0) = 0$.
The agent wishes to achieve a certain (known) threshold payoff $\threshi$ and hence,
her true demand at round
$t$ is given by $\demtrueit = \volit\payoffinvi(\threshi)$.
This implies that each agent's true demand increases proportionally with the load, with
the demand per unit load, or \emph{unit demand} for short, being $\payoffinvi(\threshi)=:\udtruei$.
We will assume that $\udtruei\in[0, \udmax]$ where $\udmax$ is known.
The agent's utility $\utili:[0, \udmax]\rightarrow\RR_+$, as illustrated in the figure to the right,
is also a function of the amount of resources allocated per unit load which increases up to
$\udtruei$, and does not increase beyond $\udtruei$.
In the figure, we have shown  $\payoffi(a) = \utili(a)$ for $a<\udtruei$,
although this is not strictly
necessary---we only require that $\utili$ be increasing up to $\udtruei$ and remain flat thereafter.

Additionally, we will make some mild assumptions so as to avoid degenerate cases in our analysis.
First, for all $i, t$,
$\volit\in (\volmin, \volmax]$ and $\sigmait \in (\sigmamin, \sigmamax]$ for some
$\volmin, \sigmamin>0$ and $\volmax, \sigmamax<\infty$; $\volmin,\volmax,\sigmamin,\sigmamax$ need
not be known.
% The lower bound conditions on $\volit,\sigmait$ are mostly for simplicity as it avoids having to
We comment more on the bounded-from-below conditions on $\volit,\sigmait$ in our proofs.
Next, we will assume $\volmax\,\udmax \leq 1$, which states that at the very least each
agent should be able to meet
their demands if they have the entire resource to themselves.
% Note that this subsumes the ``stationary'' setting described above by simply setting $\volit=1$
% for all $i,t$.
% The following example motivates the above assumptions.


\insertprethmspacing
\begin{example}[Web serving]
\label{eg:webserving}
\emph{
Continuing with the example from Section~\ref{sec:intro}, say that the SLO of each team
is to ensure that a given threshold, say $0.95$, of the queries are completed on time on average.
The load $\volit$ is the number of queries agent $i$ receives in round $t$.
Her reward $\Xit\in[0, 1]$ is the fraction of queries completed on time.
The probability each query will succeed increases with the amount of resources allocated per query;
specifically, the success of each query is a Bernoulli event with probability
$\payoffi(\allocit/\volit)$.
% We therefore have, $\EE[\Xit] = \payoffi(\allocit/\volit)$ and moreover the demand of each agent
Therefore, $\payoffi(\allocit/\volit)=\EE[\Xit]$ denotes the expected fraction of queries completed
on time.
The utility of the agent $\utili = \min(\payoffi, 0.95)$ increases with this expected fraction but
is capped at $0.95$. Hence, her demand is $\demtrueit = \volit\payoffinvi(0.95)$.
Finally, since $\Xit$ is a sum of $\volit$ bounded random variables, it is
$\sigmait=1/(2 \sqrt{\volit})$ sub-Gaussian.
In web services, it is common to set SLOs via such thresholds since the amount of resources needed
to complete all queries on time could be possibly infinite. Moreover, since the quality of the
overall  service is usually bottlenecked by external
factors~\citep{mogul2019nines}, there is
little value to exceeding such a threshold.
}
\end{example}

% \textbf{Set up:}
In an online mechanism for fair allocation with unknown demands, each agent states their threshold
$\threshi$ ahead of time.
At the beginning of each round,
each agent reports their load $\volit$ to the mechanism, then the mechanism returns an allocation
vector,
and at the end of the round each agent reports their reward $\Xit$
% (not necessarily truthfully)
back to the mechanism.
The mechanism should use this feedback to estimate demands in an online fashion and quickly converge
to an efficient ellocation in a manner that is fair and strategy-proof.
As we will see, achieving these in this setting desiderata exactly is quite challenging and hence
we will define asymptotic variants which are more suitable for our setting.

\textbf{Efficiency:}
% % First, consider efficiency.
% \emph{(i) Asymptotic Efficiency:}
We define the \emph{loss} $\LOTT$ to be the sum of resources left on the table over $T$ rounds
(recall~\eqref{eqn:lotdefn}):
\begin{align*}
% \LOTT := \sum_{t=1}^T \lot(\demtrueit, \allocit)\in \littleO(T),
\LOTT := \sum\nolimits_{t=1}^T \lot(\demtrueit, \allocit),
\hspace{0.25in}
\text{where }
\lot(\demtrueit,\allocit) \hspace{-0.02in}=\hspace{-0.02in} \min(\lotur(\allocit)
\hspace{-0.02in}+\hspace{-0.02in} \lotor(\demtrueit,\allocit),
\lotud(\demtrueit,\allocit)).
\numberthis
\label{eqn:LOTTdefn}
\end{align*}
A mechanism is \emph{asymptotically efficient} if, when all agents are reporting truthfully,
$\LOTT\in\littleO(T)$.
We will say that a mechanism is \emph{probably asymptotically efficient} if this holds with
probability at least $1-\delta$, where $\delta\in(0,1)$ is pre-specified.

\textbf{Fairness:}
% \emph{(ii) Asymptotic Fairness:}
Let $\UiT,\UeiiT$, respectively be the sum of an agent's utilities when
she participates in the mechanism truthfully for $T$ rounds, and when
she has her entitlement to herself.
Precisely,
\begin{align*}
\numberthis
\label{eqn:UiT}
\UiT = \sum_{t=1}^T \utili\left(\frac{\allocit}{\volit}\right),
\hspace{1.5in}
\UeiiT = \sum_{t=1}^T \utili\left(\frac{\entitli}{\volit}\right),
\end{align*}
A mechanism is \emph{asymptotically fair} if, $\UeiiT - \UiT \in \littleO(T)$.
% A mechanism is \emph{probably fair} if $\UeiiT - \UiT < 0$ with
% probability at least $1-\delta$, where $\delta\in(0,1)$ is pre-specified.
Similarly, a mechanism is \emph{probably asymptotically fair} if  $\UeiiT - \UiT \in \littleO(T)$
with probability at least $1-\delta$, where $\delta\in(0,1)$ is pre-specified.
% 
% To understand why we consider asymptotic fairness, observe that exact fairness can be
% trivially achieved by allocating in proportion to each user's entitlements on each round.
% But achieving an efficient allocation requires that the mechanism accurately estimates the
To understand why we consider asymptotic fairness, note that achieving an efficient allocation
requires that the mechanism accurately estimates the demands.
This is especially the case for agents whose demand is lower than their entitlement since the excess
resources can be allocated to other users who might need them.
However, in doing so, it inevitably risks allocating less than the demand and consequently violating
fairness.
Asymptotic fairness means that these violations will vanish over time.



\textbf{Strategy-proofness:}
% to allocations that are efficient and fair, and in a manner that is strategy-proof.
Let $\UiT$ be as defined in~\eqref{eqn:UiT} and $\UpiiT$ be the sum of utilities when an agent
is following any other non-truthful policy $\pi$.
% A mechanism is strategy-proof if $\UiT \geq \UpiiT$ for any policy $\pi$ for all $T\geq 1$.
A mechanism is \emph{asymptotically strategy-proof} if $\UpiiT - \UiT \in \littleO(T)$ for 
any policy  $\pi$ regardless of the behaviour of the other agents.
It is \emph{probably asymptotically strategy-proof} if this holds with
probability at least $1-\delta$, where $\delta\in(0,1)$ is pre-specified.
Finally, a mechanism is \emph{probably asymptotically Bayes-Nash incentive-compatible} if
$\UpiiT - \UiT \in \littleO(T)$ with probability at least $1-\delta$ when all other agents are
being truthful.
In the above definition, an agent may adopt a non-truthful policy $\pi$ by
misreporting her threshold $\threshi$, or on any round $t$ by misreporting
her load $\volit$ or the reward $\Xit$; in the latter case, she may be adaptive
using past information.
For example, she could inflate the mechanism's estimate of her demand by
overstating her threshold or load, or understating her rewards
with the hope of getting more resources.
A cleverer agent could potentially
 be strategic over multiple rounds, say, by incurring low utilities
in early rounds with the hope of gaining in the long run. 
% Accordingly, $\pi$ is any policy that maps an agent's past information to values
% $\.

We focus on the above notions of incentive-compatibility since 
achieving dominant-strategy incentive-compatibility can be challenging
in multi-round
mechanisms~\citep{babaioff2014characterizing,babaioff2013multi,kandasamy2020mechanism}.
Typically, authors circumvent this difficulty by adopting Bayesian notions which assume
that agent values are drawn from \emph{known} prior beliefs.
However, such Bayesian assumptions may not be realistic, and even if it were, the prior beliefs
may not be known in practice~\citep{schummer2004almost}.
In this work, we rely on notions of incentive-compatibility which hold with high probabilty and in
an asymptotic sense in order to make the problem tractable.
If a fair allocation mechanism is asymptotically truthful, the maximum utility an agent may gain by
not being truthful vanishes over time.
In many use cases, it is reasonable to assume that agents would be truthful if the benefit
of deviating is negligible.
Prior work has explored similar notions of approximate
incentive-compatibility in various mechanism design
problems~\citep{lipton2003playing,kojima2010incentives,roberts1976incentives,feder2007approximating,daskalakis2006note}
and moreover,~\citet{kandasamy2020mechanism} and~\citet{nazerzadeh2008dynamic} study asymptotic
strategy-proofness in auctions.


% The strategy-proofness requirement is straightforward to define:
% being truthful is a (weakly)
% dominant strategy for all agents, % A strategy-proof mechanism should prevent all such situations.


% Before we proceed, we note that in some use cases, strategy-proofness may not be a constraint.
% For instance, in Example~\ref{eg:webserving}, the SLOs may be set by the management, while an
% organisation's central monitoring system might be able to directly observe the load and rewards.
% Therefore, we will present two mechanisms for each feedback model.
% Both are asymptotically fair and efficient; but while the first is strategy-proof,
% the latter has better asymptotic rates.


\subsection{Feedback Models}
\label{sec:fbmodels}

All that is left to do to complete the problem set up is to specify the feedback model,
i.e., a form for the payoffs $\{\payoffi\}_i$ and the (probabilistic) model for the rewards $\Xit$.
In this paper, we will consider the following three models.

\begin{enumerate}
\item \textbf{Deterministic Feedback:}
Our first model is the simplest of the three:
all agents deterministically observe the payoff for their allocation, i.e.,
$\Xit = \payoffi(\allocit/\volit)$ on all rounds.

\item \textbf{Stochastic Feedback with Parametric Payoffs:}
Here, the rewards are stochastic, where $\Xit$ has expectation
$\payoffi(\allocit/\volit)$ and is $\sigmait$ sub-Gaussian. 
For all users, $\payoffi$ has parametric form $\payoffi(x) = \payoffthetatruei(x)
=\mu(x\thetatruei)$,
where $\thetatruei>0$ is an unknown user-specific parameter and
$\mu:\RR_+\rightarrow\RR$ is a known increasing function.

\item \textbf{Stochastic Feedback with Nonparametric Payoffs:}
Here, $\Xit$ has expectation
$\payoffi(\allocit/\volit)$ and is $\sigmait$ sub-Gaussian. 
Moreover, for all users $i$, $\payoffi$ satisfies the following for known $\Lf$,
\begin{align*}
\forall\,a_1, a_2\in [0,\udmax],\quad
\left|f(a_1) - f(a_2)\right| \leq \max\left( \left|f(a_1) - \threshi\right|,
            \; \frac{\Lf}{\udmax} \left|a_1 - a_2\right| \right).
\numberthis\label{eqn:nonparfbmodel}
\end{align*}
% Moreover,
% for all users $i$, $\payoffi$ is $(\Lf/\udmax)$--Lipschitz continuous, where
% $\Lf$ is known.
% That is,
% \[
% \forall\,a_1, a_2\in [0,\udmax],\quad
% \left|f(a_1) - f(a_2)\right| \leq 
%             \; \frac{\Lf}{\udmax} \left|a_1 - a_2\right|.
% \]
\end{enumerate}

% In this next section, we propose three different models.
% In the first, $\Xit$ is deterministically equal to $\payoffi(\allocit)$,
% in the second and third, $\Xit$ has expectation $\payoffi(\allocit)$, where $\payoffi$ belongs
% to a parametric and nonparametric family of functions respectively.

There are no additional assumptions required for the first model.
For the second model,
we chose a parametric family of the above form since it is a straightforward way to model increasing
functions, as necessitated by our problem set up.
% For instance,
In Example~\ref{eg:webserving}, an appropriate choice for $\mu$ could be $\mu(x)=\tanh(x)$
or $\mu(x) = 1 - (1+x)^{-1}$, which are bounded and increasing.
Moreover, since they are concave, they can model situations which exhibit a diminishing
returns property when more resources are allocated, as is commonly the case in
practice~\citep{venkataraman2016ernest}.
In the second model, we will assume that we know a lower bound on the parameter $\thetatruei$
and the derivative of $\mu$.
Such assumptions are common in parametric models in the online learning literature~\citep{} 
This is stated formally in Assumption\ref{asm:glm}.

\insertprethmspacing
\begin{assumption}
\label{asm:glm}
There exists known $\thetamin>0$ such that 
$\thetatruei\geq\thetamin$ for all $i$.
Moreover,
\[
\kappamudot \defeq \inf_{x\in[0,\udmax]} \frac{\ud\mu(x)}{\ud x} \geq 0.
\]
\end{assumption}

In the third model, the condition is satisfied if each payoff is 
$(\Lf/\udmax)$--Lipschitz continuous.
We will additionally require that for each user, the payoff increases sharply at
her demand, which we formalise by defining the near-threshold gradient (NTG)
of an increasing function at a point.



\insertprethmspacing
\begin{definition}[Near-threshold Gradient]
\label{def:ntg}
The near threshold gradient of a non-decreasing function
$f:\RR\rightarrow \RR$ at $\eta\in\RR$ with
$f(\eta)=\alpha$ is defined as,
\begin{align*}
% \ntg \defeq
{\rm NTG}(f, \eta) &\defeq
\sup\bigg\{G \geq 0; \; \exists \epsG>0 \text{ such that, }\;
\forall\,a\in(\eta-\epsG, \eta+\epsG),
\\  &\hspace{1.5in}
|f(x)-\alpha| \geq \,\frac{G}{\udmax}|a-\eta| \bigg\}.
\numberthis\label{eqn:nonparlipcondn}
\end{align*}
\end{definition}

\insertFigNTGIllus

If $f$ is differentiable at $\eta$, then 
${\rm NTG}(f, \eta) = f'(\eta)$.
Assumption~\ref{asm:ntg} below states that the NTG should be positive for all payoffs at their
respective demands.
To understand why such an assumption is necessary, assume that $\payoffi$ increases up to
the demand but is flat thereafter.
Then, any lower confidence bound for the payoff at any $a>\udtruei$ will necessarily be smaller
than $\threshi$ and
therefore, we will not be able to estimate this demand with any confidence.
We have illustrated this in Figure~\ref{fig:ntgillus}.
% We now state our results.

\insertprethmspacing
\begin{assumption}
\label{asm:ntg}
There exists $\ntg>0$ such that,
for all users $i$, ${\rm NTG}(\payoffi, \threshi) \geq \ntg$.
% the near threshold gradient of $\payoffi$ at $\udtruei$ 
% satisfies is at least $\ntg$
% where $\ntg>0$.
% There exists known $\thetamin>0$ such that 
% $\thetatruei\geq\thetamin$ for all $i$.
% Moreover,
% \[
% \kappamudot \defeq \inf_{x\in[0,\udmax]} \frac{\ud\mu(x)}{\ud x} \geq 0.
% \]
\end{assumption}

This completes the formulation of online learning in fair allocation.
We now present our mechanisms.



==> app_experiments.tex <==

\section{Addendum to Experiments Section}
\label{app:experiments}

We provide some details on the experimental set up.

\subsection*{Implementation Details}

For the stochastic methods, we solved for $\thetait$ in~\eqref{eqn:thetaitdefn}, by first computing
$\thetamlit$ as given in Appendix~\ref{app:glm}, and then clipping it at $\thetamin$.
However, in practice we found $\thetamlit>\thetamin$ in almost all cases.
We solved for $\thetamlit$,  using the Newton-Raphson method.

In all our experiments, we used $\delta=10^{-3}$.
We found the theoretical value for $\betat$ as given in Section~\ref{sec:glmfbmodel} to be too
conservative; therefore, we divided it by $10$.
This value was tuned using a hold-out set of synthetic experiments that were not included
in Figure~\ref{fig:synthetic}.
Note that it is common to tune upper confidence bounds in a similar manner in the bandit
literature~\citep{filippi2010parametric}.
% Note that it is common to tune upper confidence bounds in a similar manner in the bandit
% literature~\citep{kandasamy15addBO}.

\subsection*{The Prediction Serving Task}

We evaluate our approach on latency-sensitive prediction serving~\citep{crankshaw2018inferline},
which is used in a applications such as alarm systems~\cite{zhang2017live} and 
Amazon Alexa~\citep{alexa2020}.
In this setting, the user deploys a queued serving system that takes query inputs and
returns prediction responses. Due to the real-time nature of these applications, sub-second response
time is expected. This setting is of particular interest because although the application owner
knows how to quantify strict performance requirements from the application, the appropriate resource
allocation is far less clear a priori, due to the complexity of the system.

In our experiment we consider 5 such users, with equal entitlement to 100 VMs. Each
user specifies a 100ms, 0.99 percentile latency SLO target for their application response time,
meaning that they allow at most 1\% of queries in incoming traffic to have response time greater than
100ms.
At the end of each round, users provide feedback on the fraction of queries that were completed on
time.
For the arrival traffic of 3 of the users we
use varying time-of-day and day-of-week regions in the Waikato network
dataset~\citep{mcgregor2000nlanr}, for one of
them we use data from the Twitter streaming API~\citep{twitter2020},
and for one we use the Wikipedia traffic
data~\citep{wikipedia2020}.
We use a query-level execution simulator from~\citep{crankshaw2018inferline}, which uses
power-of-2-choices load balancing to mimic real deployment conditions.



==> app_nonparametric.tex <==


\section{Proofs of Theorems~\ref{thm:npsp} \&~\ref{thm:npnsp}}
\label{app:nonparametric}


